Quantifying the Quark Gluon Plasma

The study of heavy-ion collisions presents a challenge to both theoretical and experimental nuclear physics. Due to the extremely short lifetime and small size of the collision system, disentangling information provided by experimental observables and progress in physical insight requires the careful application of plausible reasoning. I apply a program of statistical methodologies, primarily Bayesian, to quantify properties of the medium in specific models, as well as compare and criticize differing models of the system. Of particular interest are estimations of the specific shear and bulk viscosities, where we find that information carried by the experimental data is still limited. In particular we find a large sensitivity to prior assumptions at high temperatures. Moreover, sensitivities to model assumptions are present at low temperatures, and this source of model uncertainty is propagated with model averaging and model mixing.

==> app2.tex <==
%\chapter{Validating Heavy-Ion Computational Models}


